From Bilingual to Multilingual Neural Machine Translation by Incremental Training

Multilingual Neural Machine Translation approaches are based on the use of task-specific models and the addition of one more language can only be done by retraining the whole system. In this work, we propose a new training schedule that allows the system to scale to more languages without modification of the previous components based on joint training and language-independent encoder/decoder modules allowing for zero-shot translation. This work in progress shows close results to the state-of-the-art in the WMT task.

==> curriculum.tex <==
In addition to using subword tokenization, we should also consider which languages to jointly train, given that their modules will be employed to train all future languages in the system. Previous multilingual architectures benefit from sharing parameters between all languages to give additional information to low resources languages during training.

In our proposed architecture this pass of information can be enforced during the training of added languages with a frozen module. Given a frozen decoder in a high resource language X $d_x$ we train an encoder for a low resource language Z $e_z$. This new encoder is not only being trained using a target network trained with more data but also it is forced to learn a representation that is compatible with the already trained one, transferring information to the low resource module. In experiments section we will show how this information from the previous training is effectively used by the new languages added to the system, to the point of outperforming the bilingual baseline for extremely low resources languages.

As for this work, all datasets belonged to the same domain and similar amounts of data were available for all languages the criterion to define the initial base system was chosen as the pair of languages that best performed in the bilingual baselines, trying to produce an initial system with the best performance.

==> discussion.tex <==
After experimentation some thoughts arise about the details of the architecture. The languages chosen for the joint training are relevant to the final performance of the system as they will be used to define the representations of the languages added later on. On the other hand as during the language addition the all weights from the joint training are frozen, independently of the order they are added the results will not vary. All added languages are independent between them.

Another aspect that surprise us during the development is the fact that the jointly trained languages have the biggest performance gap compared to the baseline system. Further research is required in this aspect, but seems plausible that while the auto-encoding task helps the systems to be compatible it may affect the performance of the translation task.

==> motivation.tex <==
\begin{itemize}
\item Current multilingual systems are based on sharing parameters over all the languages in the system
\item In order to add a new language to the system all languages have to be retrained to have a functional model
\end{itemize}
